ShapeMatcher: Self-Supervised Joint Shape Canonicalization, Segmentation, Retrieval and Deformation

In this paper, we present ShapeMatcher, a unified self-supervised learning framework for joint shape canonicalization, segmentation, retrieval and deformation. Given a partially-observed object in an arbitrary pose, we first canonicalize the object by extracting point-wise affine-invariant features, disentangling inherent structure of the object with its pose and size. These learned features are then leveraged to predict semantically consistent part segmentation and corresponding part centers. Next, our lightweight retrieval module aggregates the features within each part as its retrieval token and compare all the tokens with source shapes from a pre-established database to identify the most geometrically similar shape. Finally, we deform the retrieved shape in the deformation module to tightly fit the input object by harnessing part center guided neural cage deformation. The key insight of ShapeMaker is the simultaneous training of the four highly-associated processes: canonicalization, segmentation, retrieval, and deformation, leveraging cross-task consistency losses for mutual supervision. Extensive experiments on synthetic datasets PartNet, ComplementMe, and real-world dataset Scan2CAD demonstrate that ShapeMaker surpasses competitors by a large margin.

==> sections/1intro.tex <==
\section{Introduction}
The gradual rise of interest among researchers in generating high-quality 3D models from scans of complex scenes \cite{AUic20,MPic19,MRic19,MScv22,NRcv21,NScv22,PLcv22} has been observed in recent years.
This technology finds extensive applications in both artistic creation \cite{DAec20,JLcv21} and 3D scene perception \cite{T3cv20,H3cv21}.
Some earlier approaches \cite{WDcv19,T3cv20} involve the direct use of deep neural networks to recover 3D models from noisy scans.
However, due to the influence of noise and occlusion, recovering fine-grained geometric structures proves to be exceptionally challenging.
To address this issue, Retrieval and Deformation ($\mathbf{R\&D}$) methods\cite{JEic19,JLcv21,ASto12,DAec20,NCcv20,3Dcv19,SFni20,ROto17} have been introduced. 
Given a target input, these methods typically consist of two stages: 1) the most geometrically similar source model is selected from a pre-established 3D shape database; 2) the selected model is deformed to tightly align with the target. 
$\mathbf{R\&D}$ methods are capable of generating 3D models that incorporate fine-grained details.

\begin{figure}[t]
   \centering
   %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{images/img_1v4.pdf}
    \vspace{-0.2cm}
   \caption{\textbf{The illustration of the Neural SE(3) Invariant Embeddings.} 
   Objects obtained from real-world scans typically exhibit various poses, resulting in lack of alignment between real scans and the CAD models in the database, making it challenging to conduct an effective $R\&D$ process. 
   To address this issue, we propose the neural SE(3) invariant embedding that decouples the translation offset $T$ and rotation $R$ of the input shape, mapping them into a consistent space for meaningful $R\&D$ processes.}
   \label{fig:pre}
\vspace{-0.5cm}
 \end{figure}

However, existing $\mathbf{R\&D}$ methods often face two challenges that make them susceptible to noise and occlusion, and difficult to be practically utilized:
\textbf{1)} Current $\mathbf{R\&D}$ methods \cite{JEic19,JLcv21,ASto12,DAec20,NCcv20,3Dcv19,SFni20,ROto17,URED} assume target shapes lie in the pre-processed canonical space. 
The training and testing of the above methods are usually carried out on datasets where all shapes have been manually registered. 
When these methods are applied for inference in real world, they require manual alignment of the scanned objects or the use of additional pose estimation networks. 
However, such processes are time-consuming and labor-intensive, yielding unreliable results. 
This hinders the direct applicability of existing methods in real world. 
In contrast, aiming to yielding $\mathbf{R\&D}$ results under various observations from arbitrary poses, we employ the novel neural SE(3) invariant embeddings to implicitly align shapes at the feature level.
\textbf{2)} Previous methods \cite{JLcv21,DAec20} do not design for dealing with partially-observed shapes, making it difficult to handle cases met in real world where objects are occluded. 
Although \cite{URED} considers the partial target shapes as input in the $\mathbf{R\&D}$ process, it directly encodes the shape as a whole, which is not robust facing with heavy occlusion.
Therefore, we employ a region-weighted encoding strategy measuring retrieval tokens in part level to resist the misguidance of the occluded object parts during retrieval process.

Considering these challenges above, we introduce \textbf{I-RED}, a neural \textbf{I}nvariant matching framework for joint \textbf{RE}trieval and \textbf{D}eformation.
To ensure the matching consistency of arbitrarily posed target observations and pre-canonicalized source shapes, we propose the SE(3) decoupler to transform input target and source shapes into the same SE(3) invariant space.
Specifically, given the extracted point-cloud-based target and source features, the SE(3) decoupler initially decouples the feature offsets representing translations.
Afterwards, it embeds the rotation-equivariant cues to obtain the rotation and transform the translation-decoupled features into the neural invariant coordinate.
Finally we normalize the features in such neural invariant coordinate to decouple object scales.
Thus, the original target and source features are mapped to the SE(3) invariant space for subsequent $\mathbf{R\&D}$ process.
During $\mathbf{R\&D}$ process, another significant barrier met in real world is the partially observed target shapes. 
It brings extra difficulty to make accurate retrieval since the occluded regions in target shapes disturb the network from suitable alignment towards the full source shapes. 
Therefore, in the retrieval module, we introduce a region-weighted method, which employs a segmentation network to divide the object into semantic regions, and assesses the distance between target and source objects based on the similarity of corresponding regions.
This region-to-region measuring significantly mitigates the misretrieval caused by the inappropriate global measuring under heavy occlusion.
Finally, in the deformation stage, I-RED harnesses the offsets of the retrieval region centers between the target shape and retrieved source shape to control neural cages \cite{NCcv20} for tightly-matched deformation.

To summarize, our main contributions are:
\begin{itemize}
\item We introduce I-RED, a neural invariant matching framework for joint shape retrieval and deformation, handling partial target inputs under arbitrary poses. 
Extensive experiments on the synthetic and real-world datasets demonstrate that I-RED surpasses existing state-of-the-art approaches by a large margin.
\item We design the SE(3) decoupler network capable of extracting SE(3) invariant features to ensure the matching consistency of arbitrarily posed target observations and pre-canonicalized source shapes. 
\item We develop the region-weighted retrieval method to mitigate the impact of occlusion on the $\mathbf{R\&D}$ process.
\end{itemize}

==> sections/3method.tex <==

\begin{figure*}
   \centering
   \includegraphics[width=\linewidth]{images/pipelinev6.pdf}
   \caption{\textbf{The pipeline of I-RED.} 
   I-RED consists of two branches, namely the partial branch (A) and the full branch (D).
   Each branch includes its SE(3) decoupler for construction of neural SE(3) invariant embeddings, region segmentation network (RS) and feature extraction network (FE) for retrieval, and region center prediction (RC) network for deformation.
   The partial branch (A) takes a partial target point cloud with arbitrary poses as input, and it obtains SE(3) invariant features (B) through the branch-specific SE(3) decoupler. 
   Within the branch, the FE and RS network work together to use SE(3)-invariant features as input, generating retrieval tokens for various regions of the target (C).
   Similarly, the full branch (D) takes a full source point cloud as input, following a process similar to the partial branch, obtains region retrieval tokens for each source model.
   Subsequently, the target retrieval tokens are compared with the retrieval tokens of each source model in the database to find the nearest source model. 
   During the deformation stage, the RC network of the partial and full branch predicts region centers for the target and the retrieved source model respectively. 
   Thus, the final model is obtained through the region-center-driven cage deformation.}
  \label{fig:mid1}
  \vspace{-0.5cm}
 \end{figure*}


\section{Method}

\textbf{Overview.}
ShapeMatcher consists of 4 modules, corresponding to the 4 highly-associated tasks.
Each of the first 3 modules: \textit{Canonicalization, Segmentation} and \textit{Retrieval} modules have two parallel branches, one for complete point cloud (only used in training, in blue background) and the other for partial object input (in orange background). 
As shown in Fig.~\ref{fig:mid1}, given a partial target shape $S_{tgt}$ in an arbitrary pose, in the \textit{Canonicalization} module, we progressively decouples its inherent shape with rotation $R_{tgt} \in SO(3)$, translation $T_{tgt} \in \mathbb{R}^3$ and the $3 \mathrm{D}$ metric size $s_{tgt} \in \mathbb{R}^3$ via VN-MLP~\cite{VNic21, katzir2022vnt,chen20223gnt}, yielding the affine-invariant point-wise features $F_{tgt}$.
The object can then be canonicalized via inverse transformation based on intrinsics $\{R_{tgt}, T_{tgt}, s_{tgt}\}$.
In the \textit{Segmentation} module, $F_{tgt}$ is fed into a 4-layer MLP network to predict $M$ parts and corresponding part centers $\{K_{tgt}^1,K_{tgt}^2,...,K_{tgt}^M\}$.
The segmentation is semantically consistent across each category and thus can be matched and compared for $\mathbf{R\&D}$.
In the \textit{Retrieval} module, inside each region $M^i$, we aggregate the features of all points inside it as its retrieval token $Q^i$.
The retrieval token for the object is then represented as $\mathbf{Q_{tgt}}=\{Q_{tgt}^1,Q_{tgt}^2,...,Q_{tgt}^M\}$.
Similarly, during training, we obtain the intrinsics $\{R_{src}, T_{src}, s_{src}\}$, part centers $\{K_{src}^1,K_{src}^2,...,K_{src}^M\}$ and retrieval tokens $\mathbf{Q_{src}}=\{Q_{src}^1,Q_{src}^2,...,Q_{src}^M\}$ via the branch for complete point cloud.
By comparing $\mathbf{Q_{tgt}}$ and $\mathbf{Q_{src}}$ of each source shape inside the database, we identify the most geometrically similar source shape $S_r$.
In the final $\textit{Deformation}$ module, $K_{tgt}$ and $K_{src}$ are leveraged to guide the neural cage deformation~\cite{NCcv20} to deform $S_r$ towards $S_{tgt}$.



\subsection{Canonicalization}
As shown in Fig.~\ref{fig:mid1} (a), the \textit{Canonicalization} module takes the target point cloud $S_{tgt}$ as input and disentangle the inherent structure of $S_{tgt}$ with the intrinsics $\{R_{tgt}, T_{tgt}, s_{tgt}\}$, yielding a point-wise affine-invariant feature $F_{tgt}$. 
Specifically, we follow VN-MLP~\cite{VNic21, katzir2022vnt,chen20223gnt} to first decouple translation via VNT~\cite{katzir2022vnt} and then extract rotation via VNN~\cite{VNic21, katzir2022vnt}.
We further follow ~\cite{chen20223gnt} to normalize the SE(3)-invariant features obtained above the remove the influence of scaling, yielding $F_{tgt}$ as follows,


The SE(3) decoupler primarily uses the architecture of VN-MLP (Vector Neural Multi-Layer Perceptron) \cite{VNic21} to construct.
In the encoder, the point-cloud-based features $V \in \mathbb{R}^{N\times \eta\times3}$ \cite{VNic21} ($N$ is the number of input points and $\eta$ signifies the input feature dimension) is fed to VN-MLP to first decouple the translation $T_{tgt} \in \mathbb{R}^3$ by:
\begin{equation}
\begin{split}
  V_t = & \mathbf{VN\mbox{-}MLP}_{offset}(V) \in \mathbb{R}^{N\times1\times3}, \\
  T_{tgt} = & \frac{1}{N} {\sum}_{n=1}^N \mathbf{V_t}^{(n)} \in \mathbb{R}^{1\times3}.
  \label{eq:6}
\end{split}
\end{equation}
Following this, we subtract this translation from the original features $V' = V - T_{tgt}$ to separate the translation component.
% Decoupling the feature offsets with the feature space origin as the center enables the acquisition of accurate SO(3) equivariant features.
After decoupling the translation component, we extract the rotation-equivariant cues by $V_R = \mathbf{VN\mbox{-} MLP(V')}$. 
Then, another VN-MLP predicts the rotation matrix $R_{tgt}$ using the rotation-equivariant cues by:
\begin{equation}
  R_{tgt} = \mathbf{VN\mbox{-}MLP}_{rot}(\frac{1}{N} {\sum}_{n=1}^N V_R^{(n)}) \in \mathbb{R}^{3\times3}.
  \label{eq:7}
\end{equation}

The rotation matrix $R_{tgt}$ describes how the original input shape $S_{tgt}$ is transformed into SE(3) invariant space at the object level. At this point,  we need to extract rotation-invariant features from the rotation-equivariant cues $V_R$.

%To obtain final SE(3) invariant features, 
Following \cite{VNic21}, we create a coordinate system $T$ based on $V_R$ and then read $V_R$ within this coordinate system to generate invariant features $V_{inv} \in \mathbb{R}^{N\times C^{(inv)} \times3}$. 
Initially, we generate a matrix $T$ for each element by combining its feature $V_R$ with the overall mean feature $\bar{V}_R = \frac{1}{N} {\sum}_{n=1}^N V_R^{(n)}$. Then, we pass this matrix through a VNMLP with a target channel count of $C$ = 3:
%Initially, we generate a matrix $T_n$ for each element and subsequently apply VN-MLP with a specified target number of channels, denoted as $C = 3$.
\begin{equation}
%   T_n = \mathbf{VN\mbox{-}MLP}_{inv}([V_R^{(n)},\bar{V'}]),V'_n \in \mathbb{R}^{C\times3},
%  T_n = \mathbf{VN\mbox{-}MLP}_{inv}([V_R^{(n)},\frac{1}{N} {\sum}_{n=1}^N V_R^{(n)}]),V_R^{(n)} \in \mathbb{R}^{C\times3},
  T^{(n)} := \mathbf{VN\mbox{-}MLP}_{inv}([V_R^{(n)},\bar{V}_R]),
  \label{eq:8}
\end{equation}
after obtaining $T^{n}$, by ultimately reading $V_R$ within this coordinate system, we acquire rotation-invariant features:
\begin{equation}
  {V_{inv}}^{(n)} = V_R^{(n)}{T^{(n)}}^{\top}.
  \label{eq:9}
\end{equation}

Ultimately, we execute a flattening operation directly on the rotation-invariant features, denoted as $\hat{V}_{inv} \in \mathbb{R}^{N\times C}$.
We further decouple the scale of $\hat{V}_{inv}$ to eliminate the scale's impact on retrieval, denote as ${F^{(n)}_{tgt}} = \hat{V}_{inv}^{(n)}/\mathbf{norm}(\hat{V}_{inv}^{(n)})$.

The decoder's objective is to take $F_{tgt}$ as input and utilize the MLP along with predefined patches to reconstruct the shape $S_{tgt} \in \mathbb{R}^{N\times3}$ in the SE(3) invariant space.
We only use the decoder during the training phase to assist the network in unsupervised learning of the SE(3) invariant spatial representation, as described in detail in Sec. \ref{training}.


\begin{comment}
\textcolor{red}{\textbf{SE Training.}} 
The network learns in an unsupervised manner, encountering two main challenges throughout the learning process: 1) accurately decoupling the object's pose and predicting the object's coordinates in the invariant space, and 2) obtaining a stable representation of the invariant space.

For an object $S_{tgt} \in \mathbb{R}^{N\times3} $ with $N$ points, the encoder initially predicts its pose, denoted as $R_{tgt}$ and $T_{tgt}$. Using this pose, we transform $S_{tgt}$ into the invariant space, resulting in $S'_{tgt} = S_{tgt}R_{tgt} + T_{tgt}$. The decoder, on the other hand, employs the $F_{tgt}$ generated by the encoder to reconstruct the object in the invariant space, producing ${S'}_{tgt}^{pre}$. To achieve pose decoupling, we enforce a constraint on their Chamfer distance, represented as a loss:
\begin{equation}
  \mathcal{L}_{dec} = dis_{cham}(S'_{tgt},{S'}_{tgt}^{pre}).
  \label{eq:l1}
\end{equation}

To improve the stability of the invariant space, we introduce random rotations $R_{rand}$ and random translations $T_{rand}$ to generate $S_{tgt}^{(rand)} = S_{tgt}R_{rand}+T_{rand}$, which we then input into the autoencoder to obtain the network's predicted ${S'}_{tgt}^{pre(rand)}$. In order to further reinforce the stability of the invariant space, we impose a constraint on their Chamfer distance, expressed as a loss:
\begin{equation}
  \mathcal{L}_{stb} = dis_{cham}(S'_{tgt},{S'}_{tgt}^{pre(rand)}).
  \label{eq:l2}
\end{equation}


The total loss for training the autoencoder is given by $\mathcal{L}_{map} = \mathcal{L}_{dec}+\mathcal{L}_{stb}+orth(R_{tgt})$, with $orth(\cdot)$ serving the purpose of enforcing the orthogonality of matrices.
\end{comment}

\subsection{Region-Weighted Retrieval}
The retrieval network aims to identify the model $S_{src}$ from an existing database that bears the closest resemblance to the target object $S_{tgt}$ after deformation. 
Traditional methods \cite{URED,JLcv21} directly extract the global features of objects for retrieval, which typically suffer from heavy occlusion since the global features are susceptible to partial observation. 
In contrast, we employ a novel region-weighted retrieval method to explicitly encode independent regions of the shape. 
This allows us to accurately handle partial shapes by identifying the visible regions to retrieve models most similar to the target.
This process is jointly implemented by the region segmentation (RS) network and the feature extraction (FE) network.
We describe the retrieval module in the partial branch as an example.

\textbf{Region Segmentation.}
To obtain region feature embeddings, accurate prediction of semantic-consistent regions of the shape is required.
We achieve this using the RS network.
The RS network is modeled by a 4-layer MLP, and it takes $F_{tgt}$ as input to predict $M$ regions $F_{seg} = [C_1, C_2, C_3, ..., C_N]^\top \in \mathbb{R}^{N\times M}$ of $S'_{tgt}$, where $C_i\in \mathbb{R}^M$ represents the probability of point $i$ belonging to which class.

\textbf{Region Feature Embeddings.}
We utilize the FE network $\mathbf{MLP}_{FE}$, constructed with a 4-layer MLP, to extract features for each region. 
For more efficient computation, we employ a region aggregation approach to rapidly obtain independent features of each regions: 
\begin{equation}
  F_{cls} = F_{seg}^\top * \mathbf{MLP}_{FE}(F_{tgt}),
  \label{eq:r1}
\end{equation}
where $F_{cls} \in \mathbb{R}^{M\times C}$ contains features for each of the $M$ regions.
The region aggregation accentuate the unoccluded region of the object, so as to enhance token-matching accuracy under partial observations.
After assigning different weights to features from different regions, we can obtain the final token embeddings as follows:
\begin{equation}
  Q = F_{cls} / (\sum_{n=1}^NF_{seg}^{(n)}).
  \label{eq:r2}
\end{equation}
We use the number of points contained in each part of the segmentation as weights to balance the contribution of each region's features to the token. 
The region encoding can ignore the impact of obscured areas and instead prioritize the observed portions of the region.
In the end, the network retrieves the most similar objects by directly comparing the Euclidean distances between tokens.

\begin{comment}
\textcolor{red}{\textbf{R Training.}} 
For each training iteration, we select a shape from the dataset as $S_{tgt}$ and simultaneously choose a random model from the database as $S_{src}$. The training objectives of the retrieval network must meet two crucial criteria: 1) deformation awareness, meaning that the retrieved objects should be most similar to $S_{tgt}$ after deformation, rather than directly retrieving the most similar object to $S_{tgt}$; 2) the effectiveness of region features, implying that region features should effectively represent the similarity between $S_tgt$ and the deformed $S_src$ in the specified regions.

To achieve effective representation of region features, we directly supervise the region features, rather than supervising the entire token.

For the calculation of region feature distances to ground truth, in simple terms, we supervise the distances between tokens by computing the similarity between the deformed shape $S_{src}^{dfm}$ and the corresponding regions in $S_{tgt}$ as the ground truth for these regions. Taking the $i$-th region as an example, $S_{tgt}^i$ represents all points in $S_{tgt}$ that belong to the $i$-th region. We use $K$-nearest neighbors (KNN) to calculate the distances between each point in $S_{tgt}$ and its nearest point in $S_{src}^{dfm}$, and we take the mean of all point distances $D_i$, as the ground truth for the similarity of this region. Therefore, our region loss can be represented as:
\begin{equation}
  \mathcal{L}_{retrieval} = \frac{1}{M}\sum_{i=1}^{M}MSE(Q_{tgt}^i-Q_{src}^i,D_i).
  \label{eq:rloss}
\end{equation}
where $Q^i$ represents the token of the $i$-th region, and $MSE(\cdot)$ represents Mean Squared Error.
%\textcolor{red}{NEED ADD}
\end{comment}


\subsection{Region-Center-Driven Neural Cage Deformation}
We use the offset of the corresponding region centers of $S_{tgt}$ and $S_{src}^{sim}$ to drive the neural cage deformation.

\textbf{RC network.}
Taking the partial branch as an example, the region center prediction (RC) network $\mathbf{MLP}_{RC}$ consists of a 4-layer MLP, which is used to predict the $M$ region centers of the shape. 
Specifically, for a partial point cloud with $N$ points, the network predicts a set of region centers based on each point. 
The network aggregates the predicted $N$ sets of region centers to obtain the final $M$ region centers: 
\begin{equation}
\begin{split}
   F_{rc} & = \mathbf{MLP}_{RC}(F_{tgt}) \in \mathbf{R}^{N\times(M\times3)}, \\
   K_{tgt} & = \sum_{n=1}^N F_{rc}^{(n)} \in \mathbf{R}^{(M\times3)}.
  \label{eq:kp1}
\end{split}
\end{equation}

\textbf{Neural Cage Prediction.}
We utilize the region centers ($K_{tgt}$ and $K_{src}$) predictions for $S_{tgt}$ and $S_{src}^{sim}$ to control the vertice offsets of the neural cage for $S_{tgt}$, denoted as $C_{src2tgt}$.
In particular, we employ a neural network to predict an influence vector $I \in \mathbb{R}^{N_c \times M}$ for each point concerning all cage vertices by $I = \mathbf{MLP}(cat(F_{tgt},F_{src}))$. 
$C_{src2tgt}$ is computed through the influence vectors $I$ and the differences between region centers:
\begin{equation}
   C_{src2tgt} = C_{src} + \sum_{i=1}^M I_i(K_{src}^{(i)}-K_{tgt}^{(i)}),
  \label{eq:defo2}
\end{equation}
Finally, we employ a sparse cage scaffolding strategy \cite{NCcv20,KPcv21} to achieve the deformation of $S_{src}$. 
The deformation of $S_{src}$ can be expressed as follows:
\begin{equation}
   S_{src2tgt} = S_{src} + \Psi(C_{src},C_{src2tgt}),
  \label{eq:defo}
\end{equation}
where $\Psi$ computes the displacement of each point in $S_{src}$ by evaluating the differences between $C_{src}$ and $C_{src2tgt}$, thereby achieving deformation. 


% \textbf{Neural Cage Deformation.} We employ a sparse cage scaffolding strategy \cite{NCcv20,KPcv21} to achieve the deformation of $S_{src}$. Firstly, we initialize all vertices of the coarse control mesh of the neural cage $C_{src} \in \mathbb{R}^{N_c \times 3}$ to fully enclose the shape $S_{src}$, where $N_c$ represents the number of cage vertices. Constructing mean value coordinates \cite{NCcv20}, allows the interpolation of displacements from $C_{src}$ to any point on $S_{src}$, thus enabling deformation control over $S_{src}$. The deformation of $S_{src}$ can be expressed as follows:
% \begin{equation}
%    S_{src2tgt} = S_{src} + \Psi(C_{src},C_{tgt})
%   \label{eq:defo}
% \end{equation}
% where,  $C_{tgt}$ represents the cage vertices of $S_{tgt}$ under ideal circumstances. $\Psi$ computes the displacement of each point in $S_{src}$ by evaluating the differences between $C_{src}$ and $C_{tgt}$, thereby achieving deformation. 


\begin{comment}
\textcolor{red}{\textbf{D Training.}} 
The deformation module, similar to the retrieval module, begins by selecting a shape from the dataset as $S_{tgt}$ and randomly picking a shape from the database as $S_{src}$. We aim to learn effective deformation influence vectors $I$ and the distribution of key points $K$. \textcolor{red}{Regarding the key points $K$, their training is carried out in an unsupervised manner, in conjunction with the segmentation network, as explained in the retrieval section.} The supervision of deformation influence vectors $I$ primarily serves two purposes: 1) Supervision is applied to the influence vectors to ensure the accuracy of deformation, and 2) regularization is applied to the influence vectors to enhance the generalization of deformation.

For the accuracy of deformation, we directly achieve it by comparing the chamfer distance between $S_{tgt}$ and $S_{src2tgt}$:
\begin{equation}
  \mathcal{L}_{acc} = CD(S_{tgt},S_{src2tgt}).
  \label{eq:dloss}
\end{equation}
where $CD(\cdot)$ stands for Chamfer Distance.

So the complete deformation loss can then be expressed as:
\begin{equation}
  \mathcal{L}_{deform} = \mathcal{L}_{acc} + \Vert I \Vert_2
  \label{eq:dfloss}
\end{equation}
where we regularize $I$ using the L2 norm.
\end{comment}

\subsection{Joint Training}\label{training}
During the training phase, we train each branch network with branch-specific losses and constrain the consistency between the two branches with consistency losses.
The occlusion in input targets of the partial branch makes it challenging for the network to directly learn stable $\mathbf{R\&D}$ results.
Therefore, we employ the consistency losses by first training the full branch and then using the full branch to guide the convergence of the partial branch.

\textbf{Branch-specific Losses.} 
We train the SE(3) decoupler and the $\mathbf{R\&D}$ network in an unsupervised manner.
The SE(3) decoupler needs to decouple the input shape's pose and learn a stable representation of the SE(3) invariant space.
For an target shape $S_{tgt} \in \mathbb{R}^{N \times 3}$, the encoder computes $S'_{tgt} = C_{tgt} (R_{tgt} * S_{tgt} +T_{tgt})$. 
The decoder directly predicts $S'_{tgt}$, denotes as $\hat{{S'}}_{tgt}$. 
To achieve pose decoupling, we use chamfer distance to constrain $S'_{tgt}$ and $\hat{{S'}}_{tgt}$ by $\mathcal{L}_{dec} = dis_{cham}(S'_{tgt},\hat{{S'}}_{tgt})$.
% We apply random pose augmentation to $S_{tgt}$ to obtain $S_{tgt}^{(rand)} = S_{tgt}R_{rand}+T_{rand}$, and constrain ${S'}_{tgt}^{pre(rand)}$ with $S'_{tgt}$ to generate a stable SE(3) invariant spatial representation:
% \begin{equation}
%   \mathcal{L}_{stb} = dis_{cham}(S'_{tgt},{S'}_{tgt}^{pre}).
%   \label{eq:l2}
% \end{equation}
The total loss for training the SE(3) decoupler is given by $\mathcal{L}_{STN} = \mathcal{L}_{dec}+orth(R_{tgt})$, with $orth(\cdot)$ serving the purpose of enforcing the orthogonality of matrices.

Before the $\mathbf{R\&D}$ process, to maintain consistency between the region segmentation and the region center, we jointly train the RC network and the RS network in a self-supervised manner. 
The details can be seen in the supplementary materials.
% We first constrain the chamfer distance between key points $K_{tgt}$ and $S'_{tgt}$ to obtain meaningful key points:
% \begin{equation}
%   \mathcal{L}_{kp} = dis_{cham}(S'_{tgt},K_{tgt}).
%   \label{eq:l3}
% \end{equation}
% Simultaneously, we apply two loss functions, $\mathcal{L}_{knn}$ and $\mathcal{L}_{cs}$, to constrain the segmentation network. Loss $\mathcal{L}_{knn}$ expects to treat the points around key points as separate regions, while Loss $\mathcal{L}_{cs}$ expects each key point to be at the center of its corresponding independent region.
% So, the joint loss for keypoint extraction and segmentation network can be represented as $\mathcal{L}_{ks} = \mathcal{L}_{kp} + \mathcal{L}_{knn} + \mathcal{L}_{cs}$.
In the $\mathbf{R\&D}$ process, for an input target $S_{tgt}$, we randomly select a source model $S_{src}$ from the database for training. 
To eliminate the influence of occlusion, we do not directly use the global chamfer distance of $S_{tgt}$ and $S_{src}$ as ground truth.  
Instead, we employ a regional supervision strategy, ensuring that occluded areas do not contribute to the training of retrieval network. 
% To ensure that each region's feature is not influenced by other regions, we individually supervise each region.
%To generate region-specific feature representations more effectively, we provide individual supervision for each region.
For the calculation of ground truth, take the $i$-th region as an example. 
$S_{tgt}^i$ represents all points in $S_{tgt}$ that belong to the $i$-th region. 
We calculate the average of the nearest distances from each point in $S_{tgt}^i$ to the deformed shape $S_{src}^{dfm}$ as the ground truth token value for the $i$-th region, denotes as $D_i$. 
Therefore, our regional retrieval loss can be represented as:
\begin{equation}
  \mathcal{L}_{retrieval} = \frac{1}{M}\sum_{i=1}^{M}MSE(Q_{tgt}^{(i)}-Q_{src}^{(i)},D_i).
  \label{eq:rloss}
\end{equation}
The deformation loss is achieved by directly constraining the chamfer distance between $S_{tgt}$ and $S_{src}^{dfm}$, and it can be expressed as:
\begin{equation}
  \mathcal{L}_{deform} = dis_{cham}(S_{tgt},S_{src}^{dfm}) + \Vert I \Vert_2
  \label{eq:dloss}
\end{equation}
where we regularize $I$ using the L2 norm.

\textbf{Consistency Losses.}
If we train the partial and full branches independently, the targets and sources involved in the $R\&D$ process will not consistently lie in the same coordinate system. 
Therefore, we impose consistent constraints on the SE(3) decoupler, the RC network, and the RS network of the two branches, by first training the full branch and then using the full branch to guide the convergence of the partial branch.

During the training process, for a full input $S_{full}$, we generate a mask $U_{f2p} \in \mathbb{R}^N$ to obscure it to simulate the situation of a partial input $S_{partial} = S_{full} U_{f2p}$.
To enforce the consistency in the SE(3) invariant space between the two branches, we apply the same transformation $U_{f2p}$ to $S'_{full}$ as before and then use the chamfer distance to constrain its distance to $S'_{partial}$:
\begin{equation}
  \mathcal{L}_{cse} = dis_{cham}(S'_{partial},S'_{full} U_{f2p})
  \label{eq:rrloss}
\end{equation}
Similarly, for the consistency constraint of the RC network, we directly use the chamfer distance to constrain the region centers detected by the two branches: 
\begin{equation}
  \mathcal{L}_{key} = dis_{cham}(K_{partial},K_{full}).
  \label{eq:kloss}
\end{equation}
In the RS network, we mask the segmentation results of the full branch $F_{seg}^{(full)}$ and compare them with the results of the partial branch $F_{seg}^{(partial)}$:
\begin{equation}
  \mathcal{L}_{seg} = dis_{cham}(F_{seg}^{(full)} U_{f2p},F_{seg}^{(partial)}).
  \label{eq:seloss}
\end{equation}

\begin{comment}
For the neural invariant encoding network for partial inputs, the way it learns object poses is the same as for the full inputs. However, since partial inputs and full inputs correspond to two different networks, we need to enforce consistency in the invariant space of the two networks. This is achieved by constraining the outputs of the two network decoders using the Chamfer Distance, as follows:
\begin{equation}
  \mathcal{L}_{cn} = CD(S'_{fl},S'_{pt}),
  \label{eq:consis}
\end{equation}
where $CD(\cdot)$ stands for Chamfer Distance, $S'_{fl}$ represents the decoder output of the partial network, and $S'_{pt}$ represents the decoder output of the full network.
 Since the decoder's output represents the object's pose in the invariant space, constraining $S'_{fl}$ and $S'_{pt}$ directly ensures network consistency.

\textbf{Region-Weighted Retrieval.} 
Because partial inputs only contain a portion of the full shape, learning segmentation for partial inputs directly in an unsupervised manner is challenging. Similarly, we use the output of the full input network as the ground truth for the partial network:
\begin{equation}
  \mathcal{L}_{cr} = \frac{1}{N}\sum_{i=1}^{N}MSE(C_{fl}^i,C_{pt}^i),
  \label{eq:consis}
\end{equation}
where $N$ represents the number of points contained in the partial point cloud, and $C^i$ represents the classification vector of the $i$-th point. Through this teacher-student learning approach, the network can produce reasonable segmentation results.
\textcolor{red}{NEED ADD}

\textbf{Cage-based Deformation.}
\end{comment}

